Salience-guided Ground Factor for Robust Localization of Delivery Robots in Complex Urban Environments

In urban environments for delivery robots, particularly in areas such as campuses and towns, many custom features defy standard road semantic categorizations. Addressing this challenge, our paper introduces a method leveraging Salient Object Detection (SOD) to extract these unique features, employing them as pivotal factors for enhanced robot loop closure and localization. Traditional geometric feature-based localization is hampered by fluctuating illumination and appearance changes. Our preference for SOD over semantic segmentation sidesteps the intricacies of classifying a myriad of non-standardized urban features. To achieve consistent ground features, the Motion Compensate IPM (MC-IPM) technique is implemented, capitalizing on motion for distortion compensation and subsequently selecting the most pertinent salient ground features through moment computations. For thorough evaluation, we validated the saliency detection and localization performances to the real urban scenarios. Project page: https://sites.google.com/view/salient-ground-feature/home.

==> admin/initial_latex/0_abstract.tex <==
\maketitle

\begin{abstract}
In urban environments for delivery robots, particularly in areas such as campuses and towns, many custom features defy standard road semantic categorizations. Addressing this challenge, our paper introduces a method leveraging \ac{SOD} to extract these unique features, employing them as pivotal factors for enhanced robot loop closure and localization. Traditional geometric feature-based localization is hampered by fluctuating illumination and appearance changes. Our preference for SOD over semantic segmentation sidesteps the intricacies of classifying a myriad of non-standardized urban features. To achieve consistent ground features, the \ac{MC-IPM} technique is implemented, capitalizing on motion for distortion compensation and subsequently selecting the most pertinent salient ground features through moment computations. For thorough evaluation, we validated the saliency detection and localization performances to the real urban scenarios. 
\end{abstract}



% ==================== Backup ==============================
% In urban landscapes, particularly in areas such as campuses and towns, a multitude of custom features defy standard road semantic categorizations. Addressing this challenge, our paper introduces a method leveraging \ac{SOD} to extract these unique features, employing them as pivotal factors for enhanced robot localization. Traditional geometric feature-based localization is hampered by fluctuating illumination and appearance changes. Our preference for SOD over semantic segmentation sidesteps the intricacies of classifying a myriad of non-standardized urban features. To achieve consistent ground features, the \ac{MC-IPM} technique is implemented, capitalizing on motion for distortion compensation and subsequently selecting the most pertinent salient ground features through moment computations. For thorough evaluation, we validated the saliency detection and localization performances to the real urban scenarios. 
% ==================== Backup ==============================




%Last-mile delivery robots drive through many specific environments in complex urban areas to accomplish their missions. In such challenging environments, geometric feature based localization suffers from varying illumination and appearance changes, so robust ground features can be useful. Therefore, in this paper, we propose using \ac{SOD} to extract salient ground features and describe them to help localization more efficiently. We choose SOD instead of semantic segmentation to avoid the difficulty of classifying various customized features, which are numerous in complex urban environments such as campus and apartment complexes. To obtain consistent ground features, we apply the \ac{MC-IPM} method, which can store motion and use it for distortion compensation, and then select the optimal salient ground features through moment calculation.



==> admin/initial_latex/1_Intro.tex <==
%% ====================================================================================
%    History:
%    Date            Who         What
%    -----------     -------     -----------------------------
%    2023.08.30      hg          Init
%    2023.08.30      gh          Init
%    2023.09.12      ec          Intro에 로봇들 어떻게 citation? 
%                                Intro에 citation 추가 // unique text라는 표현??? 주용이형 << 체크 부탁 





\section{Introduction} 
% 배달 로봇은 복잡한 도시 풍경을 탐색해야 하며, 다양한 조명 조건, 역동적인 교통, 복잡한 도시 구조로 특징지어지는 시나리오에 직면하는 경우가 많습니다.
% Last-mile delivery robots need to navigate through intricate cityscapes, often facing scenarios characterized by diverse lighting conditions, dynamic traffic, and intricate urban structures

% 자율 배송 로봇이 도시 물류 시스템에 빠르게 통합되는 시대에 복잡한 도시 환경에서 이러한 로봇의 강력하고 정확한 위치 파악은 필수적인 과제가 되었습니다. 이에 따라 SLAM(Simultaneous Localization and Mapping) 기술이 발전하면서 [1, 2, 3, 4], 라스트 마일 배송 로봇이 실제로 다양한 분야에 적용되는 사례가 늘어나고 있습니다. 예를 들어 스타쉽 테크놀로지스[], 키위봇[], 누로[] 등의 기업들은 다양한 센서를 통한 환경 인식 기반의 배송 서비스를 제공하고 있습니다. 이러한 배송 로봇은 다양한 센서 구성(예: RGB 카메라, 열화상 카메라, LiDAR, RADAR, 초음파 센서, GPS 등)을 가지고 있습니다. 다양한 센서를 사용하면 로봇이 환경을 더 잘 인식할 수 있지만 배달 로봇의 비용도 증가합니다. 따라서 비전 기반 SLAM 방법은 상용화 수준의 제품 측면에서 저렴한 센서 구성을 선호하기 때문에 큰 주목을 받았습니다. 그러나 이러한 방법은 장기적으로 조명, 원근감 및 외관 변화로 인해 본질적인 한계가 있습니다. 또한 캠퍼스나 고층 빌딩이 즐비하는 도시 환경의 배송 경로는 대부분 GPS가 거부됩니다. 

% 이러한 환경에서 강력한 위치 파악을 달성하기 위해 우리는 도로 표면의 맞춤형 도로 표시에 중점을 둡니다.
% 그림 1에서 볼 수 있듯이 맞춤형 도로 표시에는 화살표, 속도 제한, 고유한 텍스트 등이 포함됩니다. 이러한 표시는 조명, 외관 변화에 덜 민감하다는 장점이 있습니다. 제안된 Localization Pipeline은 그림 1과 같다. 다음과 같은 기여가 있습니다\

% 흥미롭게도 대부분의 인공 지상 표시는 높은 가시성을 보여 인간 관찰자에게 특히 두드러집니다. 인간의 위치 파악 시스템은 종종 이러한 특징을 위상적 위치 파악의 단서로 활용합니다. 그림 1에서 볼 수 있듯이 맞춤형 도로 표시에는 화살표, 속도 제한, 고유 텍스트 등이 포함됩니다. 이러한 특성에 착안하여 우리는 SOD를 기반으로 맞춤형 지상 표시를 두드러진 지형 특징으로 포착할 수 있는 위치 파악 시스템을 제안합니다. 그림 1은 제안된 방법을 설명한다. 다른 배송 로봇이 다양한 센서 구성을 활용할 수 있지만 일반적으로 전방을 향한 단일 카메라가 사용됩니다. 제안하는 방법은 먼저 움직임 보상을 통해 단안 영상을 BEV(Bird's Eye View)로 변환합니다. 그런 다음 돌출 감지기를 적용하고 설명자 벡터의 접지 표시를 설명합니다. 마지막으로, 배달은 두드러진 지형 특징을 활용하여 포즈를 수정하고 지도에서 위치를 파악할 수 있습니다. 자세한 방법은 3장에서 설명한다. 제안하는 Localization Pipeline은 그림 1과 같다. 다음과 같은 기여를 합니다:


% contribution
% 1. 우리는 복잡한 도시 환경에서 포착할 수 있는 salient ground feature 기반으로 배달 로봇의 localization 방법을 제안합니다.
% 2. 제안된 방법은 제안된 방법은 표준 표시와 man-made marking을  ground factor로 통합합니다
% 3. 제안된 방법은 실제 캠퍼스 환경에서 밤과 낮, 그리고 다양한 지형 변화에도 경건한 성능을 보여줍니다.

% -------------------------------------------------------------------------------------------
In an era marked by the rapid integration of autonomous delivery robots into urban logistics systems, the robust and precise localization of these robots in complex urban environments has become an essential challenge. Accordingly, with advancements in Simultaneous Localization and Mapping (SLAM) \cite{campos2021orb, qin2018vins, zhang2014loam,shan2020lio} technology, last-mile delivery robots have been increasingly applied in various fields. For example, companies like Starship Technologies \cite{StarshipTechnologies}, Kiwibot \cite{Kiwibot}, Nuro \cite{Nuro}, and Neubility \cite{Neubility} provide delivery services based on environmental recognition through various sensors. % recognition or perception?
 These delivery robots have different sensor configurations (such as RGB camera, Thermal imaging camera, LiDAR, RADAR, Ultrasonic sensor, GPS, etc.). Using various sensors allows the robot to be more aware of the environment, but they also increase the cost of the delivery robot. Therefore, vision-based SLAM methods received significant attention because of the preference for low-cost sensor configurations for commercial-level products. However, such methods suffer from illumination, perspective, and appearance changes in the long term. Furthermore, delivery routes in urban environments such as campuses are mostly weak-GPS or GPS-denied regions. 


Interestingly, most man-made ground markings exhibit high visibility, making them particularly salient to human observers. Human localization systems often utilize these features as clues for topological localization. As shown in \figref{fig:main_figure}, customized road markings include arrows, speed limit, unique texts, etc. Motivated by this characteristic, we propose a localization system that can capture custom ground markings as the \ac{SGF} based on \ac{SOD}. \figref{fig:main_figure} describes the illustration of the proposed method. Even though other delivery robots may utilize a variety of sensor configurations, a forward-facing single camera is commonly used. The proposed method first converts the monocular image to the \ac{BEV} with motion compensation. Then, we apply a salient detector and describe the ground features in the descriptor vector. Finally, the delivery robot can correct the pose and localize on the map by utilizing \ac{SGF}. The details of the method will be explained in \secref{sec:3}. 


% As shown in \figref{fig:main_figure}, customized road markings include arrows, speed limit, unique texts, etc. These markings have the advantage of being less susceptible to lighting, and appearance changes. % 이러한 RM이 도심 환경에서 널리 존재한다는 것도 언급?

The proposed localization pipeline is as shown in \figref{fig:overall_system} and has the following contributions: 
\begin{itemize}
\item We propose a new salience-guided factor for loop closure and localization of delivery robots in urban scenarios. 
\item We present a robust \acf{IPM} to construct accurate ground features.
\item The proposed method incorporates salient feature detection to capture custom man-made features into the ground factors.
\item We validate our method in urban campus environments including various sequences, dynamic objects, and illumination changes. 
\end{itemize}



\begin{figure}[t] %%% t: top, b: bottom, h: here
    \centering
    \includegraphics[width=\columnwidth]{assets/main_figure/Fig1_5.pdf}
    \caption{Illustration of the proposed method. We extract and describe the salient feature on the ground from the \ac{BEV}. It can be used as a loop factor to perform localization. The below images are examples of man-made ground markings that can be easily found.}
    \label{fig:main_figure}
\end{figure}

==> admin/initial_latex/2_RelatedWorks.tex <==
%% ====================================================================================
%    History:
%    Date            Who         What
%    -----------     -------     -----------------------------
%    2023.09.04      ec          초안 작성 (첫번 째 단락) - 참고문헌 추가
%    2023.09.05      jw          초안 작성 (이후) (참고문헌 아직 안넣음)
%    2023.09.05      jw          Learning-based Road SLAM -> Ground Feature-based SLAM (참고문헌 아직 안넣음)

\section{Related Work}


\begin{figure*}[t!]
    \centering
\textit{}    \includegraphics[width=0.85\textwidth]{assets/overall_pipeline/Overall_pipeline2.pdf}
    \caption{The overall pipeline of the proposed system. The diagram describes utilizing SGF for localization and loop closure factors.}
    \label{fig:overall_system}
\end{figure*}

% There is an increasing demand for autonomous robots in recent years, and SLAM technology has been evolving in this regard \cite{mur2017orb, qin2018vins, zhang2014loam,shan2020lio}. 
% Especially, accurate localization using various sensors has been extensively studied. To achieve robust localization in complex urban environments, robots are equipped with various sensors, including Camera, LiDAR, IMU, GNSS, Wheel odometer, etc \cite{jeong2017road, lu2017monocular, suhr2016sensor}. 

% In terms of commercial-level products, low-cost sensor configurations are preferred such as cameras and IMUs.  
% Among them, vision-based SLAM methods received significant attention because of the preference for low-cost sensor configurations in terms of commercial-level product.  
% However, such methods suffer from illumination, perspective, and appearance change in the long term which are inherent limitations. To address these challenges, various methodologies utilizing readily observable Land markings such as lines and curb markers have been proposed \cite{schreiber2013laneloc, ranganathan2013light, lu2017monocular}. However, these approaches still suffer from the same limitations as they rely on traditional features. Therefore, an approach has been proposed that employs Land marking as a Ground feature \cite{jeong2017road, qin2021light}.  % 추가 


% To achieve robust localization in urban environments, robots are equipped with various sensors, including Camera, LiDAR, IMU, GNSS, Wheel odometer, etc \cite{jeong2017road, lu2017monocular, suhr2016sensor}.

% Robots are equipped with various sensors to achieve robust localization in urban environments, including RGB camera, LiDAR, IMU, GNSS, Wheel encoder, etc. 

% As mentioned above, vision-based SLAM methods suffer from illumination, perspective, and appearance changes in the long term which are inherent limitations. 
In the field of autonomous robots, precise localization is one of the most critical tasks. 
As mentioned above, vision-based SLAM methods are cost-competitive but suffer from illumination, perspective, and appearance changes in the long term.
To address these challenges, various methodologies utilizing readily observable road markings such as lines and curb markers have been proposed \cite{schreiber2013laneloc, ranganathan2013light, lu2017monocular}. 
% However, these approaches still suffer from the same limitations as they rely on traditional features.
However, these approaches still have the same limitations as relying on traditional features.
Therefore, some approaches have been proposed using ground information as ground features \cite{jeong2017road, qin2021light}.  % 추가 

% Traditional IPM techniques rely on a fixed transformation between the camera and \ac{BEV} synthetic camera, which does not work well on sloped or rough surfaces \cite{ying2016robust}.
{\bf{\ac{IPM}}}
The IPM algorithm, utilized for extracting robust ground features, is used in various applications \cite{tuohy2010distance, guo2014automatic, lin2012vision}. Traditional IPM techniques do not work well on sloped or rough surfaces \cite{ying2016robust}. To address this issue, some approaches \cite{zhang2014robust, nieto2007stabilization} use estimated vanishing points. In other works, \citeauthor{jeong2016adaptive} \cite{jeong2016adaptive} leverage camera pose information to obtain precise IPM images, introducing an extended IPM algorithm. More recently, \citeauthor{zhu2018generative} \cite{zhu2018generative} proposed a learning-based approach using synthetic datasets, while \citeauthor{bruls2019right} \cite{bruls2019right} presented a method based on real-world datasets, ensuring that IPM works well in real-world environments.


%% Ground feature-based SLAM -> Road SLAM 시작 learning based의 방법이 나왔다~
{\bf{Ground Feature-based SLAM}} Many works have leveraged ground features for robust localization in complex urban environments. Road-SLAM \cite{jeong2017road} exploits \ac{IPM} image and informative six classes of road marking that can be obtained by the machine learning approach. With the advancements in CNN-based image segmentation networks \cite{lee2017vpgnet, ahmad2017symbolic}, many approaches use this network to utilize ground features. 
The AVP-SLAM \cite{qin2020avp}, which leverages an image segmentation network \cite{ronneberger2015u} specifically trained for parking lots, enhances the accuracy of mapping and localization. \citeauthor{cheng2021road} \cite{cheng2021road} achieve efficient and accurate localization via compact semantic map with CNN-based sparse semantic visual feature extracting front-end. \citeauthor{zhou2022visual} \cite{zhou2022visual} proposed visual mapping and localization based on a compact instance-level semantic road marking parameterization.
However, these methods, relying on semantic image segmentation, suffer from pre-defined class limitation, which is unsuitable for complex and diverse environments like campuses and sidewalks. 
%% 주용이 형이 SOD 설명

%In this paper, we address localization in even more challenging environments than in earlier works. 
Delivery robots, operating in complex urban environments, face challenges such as unusual terrain (including paved roads, bumpy sidewalks, and obstacles like curbs) and dynamic occlusions from pedestrians and vehicles. They are also constrained by limitations in available sensors, including GNSS-denied scenarios and cheaper sensors. To address these problems, we introduce a \acf{MC-IPM} method in \secref{sec:3-mcipm}. We also demonstrate the extraction and utilization of undefined semantic ground features using a transformer-based \ac{SOD} model \cite{yun2022selfreformer} in \secref{sec:3-sgf-detection}, \secref{sec:3-sgf-description} and \secref{sec:3-loopclosing}.




==> admin/initial_latex/3_Method.tex <==

\section{Method}
\label{sec:3}


%! Bold -> 벡터랑 헷갈릴 수 있을 것 같음?

\subsection{Motion Compensate Inverse Perspective Mapping}
\label{sec:3-mcipm}
% mono 카메라로부터 지면 feature 취득을 용이하게 하기 위해 BEV 이미지로 투영하는 Inverse Perspective Mapping(IPM) 방법을 사용합니다. IPM은 전방 지면의 평탄함을 가정하므로 진동 상황이 잦은 환경에서는 local ground 추정을 통한 IPM 왜곡 보정이 필요합니다. 하지만 mono camera 기반으로는 local ground에 대한 추정이 어렵습니다. 이 문제를 해결하기 위해 로봇의 상대적인 움직임 변화를 측정하고 이를 통해 보정하는 후처리 프로세스인 MC-IPM을 적용합니다. 
% 먼저 IPM 보상은 pose간의 roll, pitch 차이를 이용합니다. 이전 task에서 우리는 ptich에 robust한 Adaptive ipm을 개선시켜 roll과 pitch 모두 보정이 가능한 Extended and Adaptive IPM 방법을 개발했습니다. 아래 수식을 통해 metric 단위로 변환된 pixel 좌표 (c,r)에서 camera's center coordinate (Xc, Yc, 0)으로 보정된 3D point를 투영할 수 있습니다.

% (수식)

% 식(1)은 이미지 평면에서 3d 공간으로 투영하기 전 roll 보정에 대한 작업이며 세타r은 보정될 roll 입니다. 식(2)에서 h는 카메라의 높이 fm은 metric 단위의 focal length 세타는 (수식) 입니다. 모션 변화에 대한 수식 유도 과정은 adaptive IPM에 자세히 나와있습니다. 이후 point를 다시 virtual camera로 2d projection 시켜 보상https://www.overleaf.com/project/64f03dc91ab50b5cdfff2574된 BEV image를 얻을 수 있습니다. 

% (수식)

% 여기서 extrinsic matrix는 z_c = 0을 가정하므로 차원 축소가 가능하며, K_i는 virtual camera의 intrinsic parameter입니다. IPM 투영 및 front view camera와 virtual camera의 관계는 fig. 1에서 확인할 수 있습니다. 

% 보상 작업은 다음 두 가지 상황 1)일시적인 뷸균일(예: 과속 방지턱, 균열), 2) 오르막 또는 내리막에서 주로 이루어질 수 있습니다. 로봇이 지나온 N개의 pose를 queue에 저장하고 평균을 계산합니다. 실제 주행 환경에서는 pitch 변화가 주로 발생하기 때문에 pitch 변화를 기준으로 임게값보다 큰 값은 평균 계산에 적용되지 않습니다. 이후 보정을 적용할 구간에서 평균의 상대적인 차이값을 theta_r과 theta_p를 IPM 파라미터로 넘겨줍니다. 결과적으로 로봇이 전방 N pose에 대한 지면 상황을 미리 알고 주행하는 것과 동일한 작업을 수행할 수 있습니다. 본 논문에서는 N=50 그리고 pitch 차이의 임계값은 0.025 radian으로 설정했습니다. MCIPM 보상에 대한 정성적 결과는 fig.4에 나타나 있습니다.

% -------------------------------------------------------------------------------------------
% We use the \ac{IPM} method to facilitate obtaining ground features from a monocular camera, which projects to a \ac{BEV} image

% However, it is difficult to do that based on a monocular camera. 

We use the \ac{IPM} method to facilitate obtaining ground features from a monocular camera. Since \ac{IPM} assumes that the ground in front of the camera is flat, distortion compensation through local ground estimation is necessary in environments with uneven ground. To solve this problem, we introduce \ac{MC-IPM}, a post-processing process that measures the relative motion changes of the robot and compensates for them.
%! post-processing process라는 말이 뭔가 어색

First, IPM compensation uses the difference in roll and pitch between poses. In the previous task, we improved the Adaptive \ac{IPM} \cite{jeong2016adaptive} robust to pitch and developed an Extended and Adaptive \ac{IPM} method that can compensate for both roll and pitch. 
% The pixel coordinates $(u, v)$ can be converted into meter space $(\mathrm{c}, \mathrm{r})$ and projected to the 3d point $(x_c, y_c, 0)$ of the calibrated camera center coordinates as follows
The pixel coordinates $(u, v)$ are converted into metric space $(\mathrm{c}, \mathrm{r})$ and projected to the compensated 3D point $(x_c, y_c, 0)$ of the camera center coordinates as follows

% EA IPM 인용 필요!!!!!!!
%! 이전의 task에서, 우리가? -> 뭔가뭔가
\begin{equation}\label{eqn:roll_comp}
    \left[\begin{array}{c}
    \mathrm{c}^{\psi} \\
    \mathrm{r}^{\psi} 
    \end{array}\right]=
    \left[\begin{matrix}
        \cos(-\boldsymbol{\psi})  & -\sin(-\boldsymbol{\psi}) \\
        \sin(-\boldsymbol{\psi})  &  \quad\cos(-\boldsymbol{\psi}) 
    \end{matrix}\right]
    \left[\begin{array}{c}
    \mathrm{c} \\
    \mathrm{r} 
    \end{array}\right],
\end{equation}
% \begin{align}
%     x_c &= h_c\cot(\theta'(\mathrm{r}^{\psi}) + \boldsymbol{\theta})\nonumber\\ 
%     y_c &= -X\bigg(\cfrac{\mathrm{c}^{\psi}}{f_m}\bigg)\cfrac{cos(\theta'(\mathrm{r}^{\psi}))}{cos(\theta'(\mathrm{r}^{\psi}) + \boldsymbol{\theta})}
% \end{align}


\begin{align}\label{eqn:final_ipm}
    \begin{aligned}
        x_c &= h_c\cot(\alpha + \theta'(\mathrm{r}^{\psi}) + \boldsymbol{\theta}), \\ 
        y_c &= -x_c\bigg(\cfrac{\mathrm{c}^{\psi}}{f_m}\bigg)\cfrac{\cos(\theta'(\mathrm{r}^{\psi}) + \boldsymbol{\theta})}{\cos(\alpha + \theta'(\mathrm{r}^{\psi}) + \boldsymbol{\theta})}.
    \end{aligned}
\end{align}


\begin{figure}[t] %%% t: top, b: bottom, h: here
    \centering
    \includegraphics[width=\columnwidth]{assets/mcipm_result/IPM_figure_final.png}
    \caption{Illustration of an \ac{MC-IPM} model. A corrected \ac{BEV} image is generated from a compensated 3D point projected through the \ac{MC-IPM}. The lower right example is a compensation result of a situation crossing a speed bump.}
    \label{fig:IPM_figure}
\end{figure}


\noindent \equref{eqn:roll_comp} is the roll compensation process before projecting from the image plane to 3D space, and $\boldsymbol{\psi}$ is 
the magnitude of roll change. In \equref{eqn:final_ipm}, $h_c$ is the height of the front view camera($c$), $f_m$ is the focal length in metric units, $\alpha$ is the angle between the optical axis and the ground, $\boldsymbol{\theta}$ is 
the magnitude of pitch change, and $\theta'(\mathrm{r}^{\psi})=\arctan(\mathrm{r}^{\psi}/f_m)$. The compensation formula for motion changes is detailed in \cite{jeong2016adaptive}. After that, we can obtain the compensated \ac{BEV} image by 2D projecting the 3D point to the virtual camera($\bar{c}$) through the process as,

% \noindent Equation (1) is the roll compensation process before projecting from the image plane into 3D space, and $\boldsymbol{\psi}$ is the change value of the roll. In Equation (2), $h_c$ is height of the camera, $f_m$ is the focal length in metric, $\boldsymbol{\theta}$ is the change value of the pitch and $\theta'(\mathrm{r}^{\psi})=\arctan(\mathrm{r}^{\psi}/f_m)$. The compensation formula for motion changes is guided in detail in \cite{jeong2016adaptive}. After that, we can obtain the compensated \ac{BEV} image by 2d projecting the 3d point to the virtual camera through the process as,
%! 나누기 형식 ㅁ/ㅁ이 더 보기 좋을듯


\begin{equation}
    \left[\begin{array}{c}
    x_{\bar{c}} \\
    y_{\bar{c}} \\
    1
    \end{array}\right]=    
    \left[\begin{matrix}
        0 & -1 & 0 \\
       -1 &  0 & X_c \\
        0 &  0 & Z_c
    \end{matrix}\right]
    \left[\begin{array}{c}
    x_c \\
    y_c \\
    1
    \end{array}\right],
\end{equation}


\begin{equation}
    \left[\begin{array}{c}
    u_{\bar{c}} \\
    v_{\bar{c}} \\
    1
    \end{array}\right]=\mathbf{K_{\bar{c}}}
    \left[\begin{array}{c}
    x_{\bar{c}} \\
    y_{\bar{c}} \\
    1
    \end{array}\right],
\end{equation}
%
 where  $(X_c,0,Z_c)$ and $\mathbf{K_{\bar{c}}}$ are position(camera center coordinates) and intrinsic parameters of virtual camera, respectively. The \ac{IPM} projection and the relationship between the front view camera and the virtual camera are shown in \figref{fig:IPM_figure}.
% ipm이 지면의 평탄함을 가정하는것이므로, it -> IPM ?

Compensation can be applied primarily in two cases: 1) temporary unevenness (e.g., speed bumps, cracks) and 2) uphill or downhill, as shown in \figref{fig:IPM_figure}.
First, store ${N}$-poses in a queue and calculate the average. 
% In driving situations, pitch changes occur mainly, so values larger than the threshold based on pitch changes do not included to the average calculation.
Since pitch motion change mainly occurs in driving scenarios, the average calculation does not include poses greater than the pitch threshold. % valus가 정확히 어떤 의미?
Subsequently, the relative difference between the average pose in the area and the robot's pose that needs to be compensated is passed as \ac{IPM} parameters $\boldsymbol{\psi}$ and $\boldsymbol{\theta}$. As a result, the robot can drive in the same way as it knows the ground situation for the front $N$-poses. In this paper, we set the threshold for $N=50$ and pitch differences, $d_{\boldsymbol\theta}=0.025$ radians. The qualitative result for \ac{MC-IPM} compensation as shown in \figref{fig:IPM_figure}.
%! In driving situation




%\begin{figure}[t] %%% t: top, b: bottom, h: here
%    \centering
%    \includegraphics[width=\columnwidth]{assets/mcipm_result/MCIPM_results1.png}
%    \caption{Illustration of \ac{MC-IPM} Compensation Results in various distortion situations.}
%    % IPM과 MC-IPM을 적용했을 때 방지턱과 오르막, 내리막 앞에서의 결과 이미지. MC-IPM을 적용하였을 때 기존에 대응할 수 없었던 경우에도 IPM이 잘 되는 것을 볼 수 있음.
%    \label{fig:mcipm}
%\end{figure}

% 주요 상황에 따른 MCIPM 보상 결과.



% ============================================================================================
% 이름 바꿀 필요가 있어보임
\subsection{Salient Ground Feature Detection}
\label{sec:3-sgf-detection}
% 지면의 salient feature를 추출하기 위해 transformer 기반의 SelfReformer 모델을 사용했습니다. Salient object detection task의 domain은 지면 feature와 거리가 있는 점을 고려하여 약간의 경향성 부여을 위해 추가 학습을 진행했습니다. 추가 학습 데이터는 SeRM-Dataset (3811 images)을 사용하였으며 validation은 4:1 비율로 분할하였습니다. 학습에 사용된 road marking들은 일반적인 차도에서 주로 볼 수 있는 arrow, diamond, speed limit 등으로 구성되어 있습니다. 배달 로봇이 주행하는 환경 특성상 customized feature와 standard feature가 같이 존재하기 때문에 두 feature를 포함해서 최대한 많은 feature를 뽑을 수 있습니다. 
% SelfReformer의 input은 MC-IPM으로 보정된 BEV image (3-channel) 이고  Salient mask (1-channel)를 output으로 얻습니다

% -------------------------------------------------------------------------------------------
In the general computer vision field, salient object detection (SOD) targets the segmentation of foreground objects in normal scenes. Motivated by this approach, we utilize general \ac{SOD} networks to capture representative ground features. For \ac{SGF} extraction, we adopt a SelfReformer\cite{yun2022selfreformer} network, a transformer-based model. However, the general SOD networks show difficulties on ground features. Therefore we re-design the training sets with a partial mixture of well-known road markings (such as arrows, diamonds, speed limit, etc.). To this end, we re-formulate SelfReformer into SelfReformer* that can capture the characteristics of salient ground features. The input of the SelfReformer* is the BEV image (3-channel) calibrated by MC-IPM and the salient feature mask (1-channel) is obtained as the output.


%Considering that the domain of the \ac{SOD} task is far from the ground features, we performed additional training to give it some tendency. To this end, we used SeRM Dataset (3811 images) classified into several road markings and, the validation is split 4:1. The road markings used in the training consist of arrows, diamonds, speed limit, etc. Due to the environmental nature of the delivery robot, customized features and standard features exist together, so we can integrate various features into localization by covering both cases.
%! 4:1이 어떤 건지 좀 더 자세하게 설명 필요할 것 같음.
%! 마지막 2개의 문장이 잘 연결되지 않는 느낌




% ============================================================================================
% 앞선 과정으로 binary feature mask를 얻으면 binary image의 특징을 capture할 수 있는 Image moment를 기반으로 optimal한 feature를 선택하여 가장 유의미한 SGF를 추출할 수 있도록 합니다. 모든 query image에 대해 extraction을 수행하기 보다는 가장 유의미한 feature를 detection하여 선택적으로 추출하는 것이 효율적입니다. 이는 온전히 등장하지 않은 feature를 SGF로 정의하게 되는 모호함을 방지할 수 있습니다. 

% moment based detector는 sliding window 기법으로 총 4가지 step에 걸쳐 optimal한 SGF를 detection합니다. 우선 feature가 나타나는 시점부터 사라지는 구간인 valid feature range를 결정합니다. 그 다음 valid feature range에 존재하는 모든 feature에 대해 Hu moment를 계산합니다. Hu moment의 각 요소는 translation과 scale에 robust한 특성을 가지는 \eta로 구성되어 있으며 아래와 같습니다. 

% (수식)

% 여기서 f(.)=I(x,y)로 intensity를 나타내며 i,j는 moment의 차수입니다. 그리고 \mu는 central moment로 tranlation에 불변한 특성을 가지며 \eta는 0차 central moment를 통해 central moment를 정규화 하여 얻어집니다. Hu moment는 translation, scale, rotation에 불변하며 아래와 같이 계산합니다.

% (수식)

% 여기서 V는 valid feature range에 속한 모든 set이며 Hu moment의 7가지 성분은 [cite]를 따릅니다.

% 이후 hu moment을 이용한 shape matching을 통해 현재 feature와 이전 feature와의 I2 distance를 계산합니다.
% 마지막으로 distance가 임계값(=0.005)보다 가까운 그룹 내에서 최적의 feature를 선택합니다.
% hu moment의 3가지 불변 속성으로 연관성이 높은 연속적인 feature를 catch할 수 있으며 마지막 그룹 내에서 가장 salient가 두드러진 feature를 최적의 feature로 선택합니다. 또한 feature 영역이 이미지의 네 경계를 벗어나면 optimal feature로 선택하지 않습니다.

% \subsection{Moment based Salient Ground Feature Detection}

After obtaining the binary salient feature mask in the previous step, we select the optimal \ac{SGF} based on the image moment that can capture the nature of the binary image. Rather than performing extraction for all query images, we perform an efficient way that extracts the most significant features. This also avoids the ambiguity of defining a feature as an SGF that has not fully appeared. 


The moment-based detector uses a sliding window approach to find the optimal \ac{SGF} in 4-steps. 1) First, it determines the valid feature range, which is the range from when a feature appears to when it disappears. 2) Then, it calculates the Hu moment\cite{1057692} for all features in the valid feature range. Each element of the Hu moment consists of $\eta_{ij}$, which has robust properties in translation and scale, as follows,
%! step 4개가 뭔지 한번에 말한다음에 하나씩 하는게 좋을 것 같음 -> 1) 2) 3) 4)의 간격이 너무 김


% i는 valid range내의 모든 index
% 수식을 구체적으로 어떻게 할지 정리 필요
\begin{equation}
    \mu _{{pq}}=\sum _{{u\in U}}\sum _{{v\in V}}(u-{\bar{u}})^{p}(v-{\bar{v}})^{q}I(u,v),
\end{equation}

\begin{equation}
    \eta _{{pq}}={\frac  {\mu _{{pq}}}{\mu _{{00}}^{{\left(1+{\frac {p+q}{2}}\right)}}}},
\end{equation}

\noindent where $I(\cdot,\cdot)$ represents intensity at pixel coordinates $(u, v)$, and $p$,$q$ is the order of moment. In addition, $\mu_{pq}$ is the central moment, which is invariant to translation, and $\eta_{pq}$ is obtained by normalizing the central moment through the zero-order central moment. The Hu moment $\mathcal{H}$ is calculated to be invariant to translation, scale and rotation as follows.
 

% \begin{equation}
% \mathcal{H}_i=\{{}^{i}h_1, {}^{i}h_2, \ldots, {}^{i}h_7\}, \quad i\in \mathcal{V}.
% \end{equation}

\begin{equation}
\mathcal{H}_i=\{h_i^1, h_i^2, \ldots, h_i^7\}, \quad i\in \mathcal{V}
\end{equation}


\noindent where $\mathcal{V}$ is all sets in a valid feature range, and the seven components of Hu moment follow \cite{1057692}. 3) Next, we calculate the distance between the current feature and the previous feature by shape matching using the Hu moments as follows, 

% % shapematching 수식
% \begin{equation}
% d_{hu}(\mathcal{H}_{i-1}, \mathcal{H}_{i})=\sum_{j=1}^7\left|{}^{i-1}h_j - {}^{i}h_j\right|
% \end{equation}


\begin{equation}
d_{hu}(\mathcal{H}_{i-1}, \mathcal{H}_{i})=\sum_{j=1}^7\left|h_{i-1}^j - h_i^j\right|, \quad i\in \mathcal{V}.
\end{equation}


% Moment based detector figure
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{assets/sgf_detector/SGF_detector.png}
    \caption{An example of a \ac{SGF} detected in a valid feature range. In the above case, two SGFs were detected in the three final groups, and not selected in final group 2 because the salient region is not included within the image boundary.}
    \label{fig:detector}
\end{figure}


\noindent Finally, 4) we select the  the group's most salient feature whose distance is closer than the threshold (=0.005). If the feature region is outside the four boundaries of the image, we do not select it. According to the three invariant properties of Hu moment, it can catch consecutive features that are highly correlated. An example is shown in \figref{fig:detector}.





%==================================================================================================
\subsection{Salient Ground Feature Description}
\label{sec:3-sgf-description}
% Optimal SGF가 선택되면 salient 영역을 3D 공간으로 아래와 같이 extraction 합니다. 

%(수식)

% 이후 SGF point에 대해 voxelization을 진행합니다. SGF를 loop factor로 사용하기 위해 3d 공간으로 투영된 SGF points에 대한 descriptor를 생성합니다. feature를 다양한 각도에서 볼 수 있는 상황과 reverse loop를 달성하기 위해 회전에 강건한 description인 scan context에서 제안된 방법을 채택했습니다. SGF points의 centroid를 중심으로 L_max 거리 내부에 대해 방위각 및 반경 방향으로 빈을 분할합니다. 본 논문에서는 ground feature의 평균적인 크기를 고려하여 Lmax = 2로, reverse loop closing을 위해 rotation에 조금 중점을 두어 N_s = 90, N_r = 10으로 사용했다. Description 과정은 fig에 나타나 있습니다.

% SGF descritor는 온라인 clustering을 통해 다양한 Feature로 group화 됩니다. Query SGF descriptor %Dq$가 결정됐을 때, 이전 SGF group의 Descriptor $Dg$와 아래와 같이 cosine similarity를 통해 가장 가까운 SGF group으로 할당됩니다.

% (수식)

% 여기서 cq, csg는 각각 query와 sg의 j번째 column이고 Nc는 전체 column의 개수입니다.
% 이후 Dg는 group의 속한 D의 평균으로 대체됩니다. 만약, 모든 Dg와의 similarity가 70보다 작다면 새로운 SGF group으로 할당됩니다. Clustering 전략은 algorithm 1에 나타나 있습니다.
% ---------------------------------------------------------------------------------------------


Once the optimal \ac{SGF} is selected, those regions are extracted into 3D space as follows,

\begin{equation}
    \left[\begin{array}{c}
        x_{sal} \\
        y_{sal} \\
        1
    \end{array}\right]=    
    \left[\begin{matrix}
        0 & -1 &  0 \\
       -1 &  0 & X_c \\
        0 &  0 & Z_c
    \end{matrix}\right]^{-1} \cdot \mathbf{K_{\bar{c}}}^{-1}
    \left[\begin{array}{c}
        u_{sal} \\
        v_{sal} \\
        1
    \end{array}\right],
\end{equation}



\noindent Afterward, voxelization is performed for \ac{SGF} points. To use the SGF as a loop factor, we create a descriptor for the \ac{SGF} points. We adopted the method proposed in scan context\cite{8593953}, which is a rotation robust description. Splits bins in azimuth and radial directions within the $L_{max}$ around the centroid of the \ac{SGF} points. In this paper, we used $L_{max}=2$, considering the average size of the ground feature. To perform a reverse loop closing, we set $N_s=90$, a central angle ($2\pi/N_s$), and $N_r=10$, a radial gap($L_{\max }/N_r$). The description process is shown in \figref{fig:description}.

And then, \ac{SGF} descriptors are grouped into various features through online clustering. When the query \ac{SGF} descriptor $\mathcal{D}^q$ is determined, it is assigned to the closest group via cosine distance to the previous \ac{SGF} group's descriptor $\mathcal{D}^{sg}$ using column shifting as follows, 


 \begin{equation}
     d(\mathcal{D}^q, \mathcal{D}^{sg}) = \frac{1}{N_c}\sum_{j=1}^{N_c} \left(1 - \frac{c_j^q \cdot c_j^{sg}}{\lVert c_j^q \rVert \lVert c_j^{sg} \rVert}  \right ),
\end{equation}


\noindent where $c_j^q$ and $c_j^{sg}$ are the j-th columns of $\mathcal{D}^q$ and $\mathcal{D}^{sg}$, respectively, and $N_c$ is the number of columns.
$\mathcal{D}^{sg}$ is then replaced by the mean of $\mathcal{D}$ in the group and is then used for comparison with the new $\mathcal{D}^q$. If the distance with all $\mathcal{D}^{sg}$ is greater than 0.7, it is assigned as a new \ac{SGF} group. 
% The clustering strategy is shown in algorithm 1.

% \begin{algorithm}
%     \caption{C}
%     \label{c4.5}
%     \begin{algorithmic}
%             \Require{Current SGF descriptor $\mathcal{D}$}
%             \Ensure {\ac{SGF} group ID for current SGF descriptor}
%             \If {$D$ is “pure” OR other stopping criteria met}
%             \State{terminate}
%             \EndIf
%       \ForAll {attribute $a$ $\in$ $D$}
%             \State {Compute information-theoretic criteria if we split on $a$}
%             \EndFor
%             \State {${a}_{best}$ = Best attribute according to above computed criteria}
%       \State {${Tree}_{v}$ = Create a decision node that tests ${a}_{best}$ in the root}
%       \State {${D}_{v}$ = Induced sub-datasets from $D$ based on ${a}_{best}$}
%       \ForAll {${D}_{v}$}
%       \State {${Tree}_{v}$ = C4.5(${D}_{v}$)}
%       \State {Attach ${Tree}_{v}$ to the corresponding branch of Tree}
%       \EndFor
%       \
%       \Return Tree
%     \end{algorithmic}
% \end{algorithm}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{assets/description/description.pdf}
    \caption{Illustration of \ac{SGF} description process and rotational invariance through column-shifted matching. The red dot is the center of the \ac{SGF} points, and the green circle is the radius $L_{max}$ boundary.}
    \label{fig:description}
\end{figure}




%==================================================================================================
\subsection{Loop Closing with SGF Factor}
\label{sec:3-loopclosing}
% 로봇이 같은 SGF가 있는 구간을 다시 주행할 경우 SGF간 association을 통해 SGF loop closing을 수행할 수 있습니다. SGF가 선택되어 SGF group이 결정되면, 그룹 내에서 가장 가까운 descriptor와 icp matching을 수행합니다. 만약 reverse 상황이라면 가장 가까운 descriptor를 찾을 때의 best column을 이용하여 icp initial을 줄 수 있습니다. SGF loop closing 통한 global pose graph optimization은 아래와 같습니다.

% 수식

% 여기서 x={}고 
% ---------------------------------------------------------------------------------------------

When the robot re-visits an area with the same \ac{SGF}, loop closing can be performed via \ac{SGF} association. Once \ac{SGF} is selected and the SGF group is determined, perform the \ac{ICP} matching with the closest descriptor within the group. In the reverse loop situation, we can provide the \ac{ICP} initials using the best column key obtained when computing the nearest descriptor. \ac{SGF} groups with symmetric properties (e.g., manhole) are excluded from loop \ac{SGF} because they cannot provide an accurate pose as a result of \ac{ICP}. The global pose graph optimization with \ac{SGF} loop factor is as follows,

\begin{align}
    \begin{aligned}
         \mathcal{X}^*= \underset{\mathcal{X}}{\operatorname{arg}\min} \sum_{t} \lVert f(\mathbf{x}_t,\mathbf{x}_{t+1})-\mathbf{z}_{t,t+1} \rVert^2_{\Sigma_t} \\
         + \sum_{i,j\in \mathcal{L}} \lVert f(\mathbf{\mathcal{S}}_i,\mathcal{S}_{j})-\mathbf{z}_{i,j} \rVert^2_{\Sigma_{ij}},
    \end{aligned}
\end{align}

\noindent where $\mathbf{x_t}=\left[\mathbf{r}_t,\mathbf{t}_t \right]^T$ is the camera pose at $t$, $\mathcal{X}=\left[\mathbf{r}_0,\mathbf{t}_0, \ldots ,\mathbf{r}_t,\mathbf{t}_t\right]^T$ are all sequences, and $\mathbf{z}_{t,t+1}$ are relative pose between   camera frame at $t$ and $t+1$. $\mathcal{S}_i$ and $\mathcal{S}_j$ are \ac{SGF} pairs observed in different sequences and $\mathcal{L}$ is a set of all \ac{SGF} loop pairs. The function $f(\cdot,\cdot)$ estimates the relative pose.

==> admin/initial_latex/4_Results.tex <==
%% ====================================================================================
%    History:
%    Date            Who         What
%    -----------     -------     -----------------------------
%    2023.09.05      jw          MC-IPM result figure template
%    2023.09.07-08      ec       Metrics and qualitative result of SOD Algs.
%                                => 수정할 사항 : SOD 결과를 6장의 이미지에서 얻은 결과를 평균낸것인데, 6장으로 결과 

\section{Experimental Results}

\subsection{Experimental Setups}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.82\columnwidth]{assets/etc/nub_scout_v2.png}
    \caption{Robots were used in the experiments. (Left) A delivery Robot from Neubility \cite{Neubility}. (Right) A 4-wheeled Mobile Robot.}
    \label{fig:robot}
\end{figure}

In the experiments, we utilized two mobile robots: A real delivery Robot from Neubility \cite{Neubility} and a general 4-wheeled mobile robot. \figref{fig:robot} represents the robots and sensors for evaluation. Both robots are equipped with wheel encoder, RGB camera, IMU sensor and a 64-channel LiDAR. We manually constructed the ground-truth trajectories using well-known LiDAR SLAM methods \cite{xu2021fast, kim2022lt}. All the measurements were recorded on Intel NUC (Intel i7, 64GB RAM, 4.7 GHz).   % ( \hl{add details such as  3.X Ghz or model name)}.
 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\columnwidth]{assets/setup/seq3.pdf}
    \caption{Test environments. The title of each dataset and legend of trajectories indicate the type of the sequence. Also, each map figure includes some representative markings.}
    \label{fig:seq_info}
\end{figure}

As described in \figref{fig:seq_info}, test sequences are composed of various driving scenarios on a campus because a campus environment includes many dynamic objects such as people and vehicles. Also, to evaluate the long-term operation, we evaluated the proposed method for the night sequences. \textit{Seq. Delivery} assumes a delivery route. In this scenario, the robot performs a delivery mission and then returns to its home. \textit{Seq. Reverse+Slope} is a scenario where all loops are reverse loops only. \textit{Seq. Large loop} covers about 2.7 kilometers, including both forward and reverse loops. %Furthermore, to evaluate the localization performance in an environment with illumination and appearance changes, \hl{additional} was acquired along the same path in the early morning. 
For the concrete evaluation, we tested the proposed method in terms of saliency detection performance, feature detector score, and localization accuracy. 

% 실험 설명이 필요합니다. 어떤어떤 테스트를 했다. 

% \figref{fig:seq_info}에서는 취득한 시퀀스에 대한 경로와 해당 경로에 존재하는 man-made land marking의 예시를 보여줌. 모든 시퀀스는 오후 3시 정도의 캠퍼스 환경에서 데이터 취득을 진행하였음. 이 환경은 사람이나 차와 같은 동적물체가 매우 많고, 건물 이나 조경에의해 생기는 그림자 때문에 illumination 변화가 어느정도 있는 환경이었음. big loop sequence는 총 2106.003초 동안 2781.174m의 거리를 가지고 있으며, 새벽 2시에 밤 환경에서의 똑같은 루트를 주행하였음. reverse loop sequence는 오직 reverse loop만을 가지고 있는 시퀀스이며 1616.628m path length, 1263.208s duration, 마지막으로 delivery sequence는 실제 로봇의 배달상황을 가정하여 출발후 목적지를 지나 다시 원 위치로 돌아오는 시나리오임. 

% 우리가 제안하는 SGF factor의 효율성을 보여주기 위해, 우리는 전통적인 sparse feature 와 IMU 기반의 ORB-SLAM3방법과

%  Among the experimental results, it is noteworthy that the proposed method exhibits robust localization performance in challenging environments where traditional visual SLAM algorithms often fail(e.g Localization in multi-session environments spanning both day and night).
% The Proposed method was able to achieve 123123123 result  of 2222222222222 route, and 33333 accuracy.

 % ======================================== Metric ========================================== => sod 관련 metric 외에도, 다른 ATE 같은 Metric 설명 필요?
% % \noindent \textbf{\textit{A. Metrics}}
% \subsection{Metrics and Evaluation Criteria}


%% ==== SOD Resllt ==============================================================
\subsection{Salient Object Detection}

To test the performance of SelfReformer*, we compared the method to the well-known SOD networks \cite{wei2020label, qin2020u2} and the foundation model of semantic segmentation (GroundedSAM \cite{groundedSAM}). We reformulated the training sets by combining DUTS-TR \cite{wang2017} and SeRM \cite{jang2021lane} to achieve generalities of saliency detection and domain adaptation to the ground features. In \figref{fig:sod_result}, SelfReformer* shows the best performance on saliency mask prediction. This result reports the validity of the training sets for man-made ground markings. Also, we found an interesting point on the result of GroundedSAM. Although GroundedSAM is known for great generality on visual perception, only some parts of the custom man-made markings can be represented by pre-defined semantics. On the other hand, SelfReformer* recognizes salient objects without pre-defined class information, so it can effectively recognize man-made features as well as standard markings in BEV images. For quantitative evaluation, we evaluated performance using well-known metrics (MaxF($F_m$), MAE($M$), MeanF($F_A$), S-measure($S_m$) on the SOD task \cite{chen2018reverse, wei2020label, pang2020multi, wei2020f3net}. As shown in \tabref{tab:sod_result}, Self-Reformer* outperforms all other methods in terms of F-measure, MAE and S-measure. (The best results are highlighted in bold.)
% https://www.overleaf.com/project/64f03dc91ab50b5cdfff2574


\begin{figure}[t!]
\centering
% \includegraphics[width=0.40\textwidth]{assets/sod_result/final_sod_result.png}
\vspace{-6.0em}
\includegraphics[width=1.0\columnwidth]{assets/sod_result/sod_final_v3.pdf}
\vspace{-7em}
\caption{\ac{SOD} results. Quantitative comparisons between SelfReformer* (Ours) and other SOD networks. We also test GroundedSAM for the ground feature segmentation.}
\label{fig:sod_result}
\end{figure}


%present the quantitative prediction results of three SOD networks and one segmentation network for both standard marking and man-made features.

%As previously mentioned, we utilized SOD Networks considering the distinctiveness of the man-made feature.
% As can be seen in , We present qualitative prediction results of three SOD networks and one segmentation-based networks on
%In \figref{fig:sod_result}, we present the quantitative prediction results of three SOD networks and one segmentation network for both standard marking and man-made features. We utilized the Grounded-SAM Network to compare segmentation-based network with SOD-based networks.
%Grounded-SAM is a foundation model that performs instance-level segmentation by combining the recently published Grounding DINO \cite{liu2023grounding} and Segment-Anything \cite{kirillov2023segment}. Due to its ability to learn generalized data representations, Grounded-SAM seems to achieve precise segmentation even for man-made markings that have not been observed previously. However, in the case of the right turn marking, Grounded-SAM recognizes it as two different objects. The ground is also incorrectly detected as a road marking. On the other hand, Salient object detection recognizes salient objects without pre-defined class information, so it can effectively recognize man-made features as well as standard markings in BEV images.



\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.1} 
\resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{l | c | c | c | c}
    \toprule
        {Methods}
        & {$F_m\uparrow$}   % 아래첨자 
        & {M\,$\downarrow$}
        & {$F_A\uparrow$}
        & {$S_m\uparrow$}
        \\
        \hline\hline
        
        % \bf{SelfReformer*}       & {\bf{.923}}  & {\bf{.006}}  & {\bf{.880}} & {\bf{.960}}    \\
        % \bf{SelfReformer}        & {.675}       & {.028}       & {.402}      & {.544}    \\
        % \bf{LDF}                 & {.495}       & {.036}       & {.440}      & {.595}    \\
        % \bf{U2Net}               & {.625}       & {.027}       & {.605}      & {.789}    \\
        
        SelfReformer*   & {\bf{.953}}  & {\bf{.032}}  & {\bf{.908}} & {\bf{.920}}    \\
        SelfReformer\cite{yun2022selfreformer}  & {.463}       & {.259}       & {.310}      & {.575}         \\
        LDF \cite{wei2020label}    & {.545}       & {.179}       & {.422}      & {.664}         \\
        U2Net \cite{qin2020u2}  & {.580}       & {.140}       & {.565}      & {.679}         \\
        
        
    \bottomrule
    \end{tabular}
}
\newline\textbf{}
\caption{Quantitative comparisons SOD performance.}
\label{tab:sod_result}
\end{table}




%On the other hand, SOD networks excel at recognizing both standard and man-made ground features.


% '또한, mobile robot은 제한적인 Computing resource를 가지기 때문에' , ==> 해당 내용 추가 안해도 되겠지 ? 당연한 말인것 같아서.
% the segmentation-based network\cite{} struggles to recognize man-made ground features that has not been learned previously.





\subsection{Localization Evaluation}
We present experimental results to validate the performance of the proposed auxiliary factor in the localization system. Since our algorithm is a vision-based localization method using both standard and man-made features in a complex urban environment, it is hard to compare directly with existing algorithms. Thus, we compared the results with Odometry and ORB-SLAM3. In ORB-SLAM3, we used a Monocular-IMU system to avoid scale ambiguity and manually perform scale correction on the outputs. We used evo \cite{grupp2017evo} to estimate \ac{ATE}.

% 우리는 SGF를 보조 factor로 사용했을 때의 효과를 확인하기 위해 Odometry와 ORB-SLAM3에 SGF factor를 추가한 결과를 비교해 보았음. ORB-SLAM3에서 우리는 scale ambiguity를 피하기 위해 Monocular-IMU 시스템을 이용했고, 최종 결과를 manually scale correction을 수행하였다. 우리는 evo를 이용해 APE와 RPE를 측정을 수행하였음.

\begin{figure}[t] %%% t: top, b: bottom, h: here
    \centering
    \vspace{-3mm}
    \includegraphics[width=1\columnwidth]{assets/traj_figure/trajectory2.pdf}
    % \subfigure[Seq. Large Loop]{%
    %     \includegraphics[width=0.45\columnwidth]{assets/traj_figure/bigl--.pdf}
    %     \label{fig:traj_plot:seq_lloop}
    % } 
    % \subfigure[Seq. Large Loop (Night)]{%
    %     \includegraphics[width=0.45\columnwidth]{assets/traj_figure/nbigl--.pdf}
    %     \label{fig:traj_plot:seq_night_lloop}
    % } 
    % \subfigure[Seq. Reverse + Slope]{%
    %     \includegraphics[width=0.45\columnwidth]{assets/traj_figure/reve.pdf}
    %     \label{fig:traj_plot:seq_reverseloop}
    % } 
    % \subfigure[Seq. Delivery]{%
    %     \includegraphics[width=0.45\columnwidth]{assets/traj_figure/deli.pdf}
    %     \label{fig:traj_plot:seq_delivery} 
    % }
    \vspace{-2mm}
    \caption{Results of adding \ac{SGF} factor with each sequence in campus scenario. Best viewed in color. }
    \label{fig:traj_plot}
\end{figure}

\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.1} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|r|r|r|r}
    \toprule
    \multirow{3}{*}{Methods}  &    \multicolumn{4}{c}{\bf{Sequence.}}
    \\ 
    \hline
     & \multicolumn{1}{c|}{Large Loop} 
     & \multirow{2}{*}{Reverse + Slope} 
     & \multirow{2}{*}{Delivery} 
     & \multicolumn{1}{c}{Large Loop }
    \\
     & \multicolumn{1}{c|}{(Day)}
     & 
     & 
     & \multicolumn{1}{c}{(Night)}
    \\\hline\hline
    Odometry    
        & {292.966}
        & {140.532}  
        & { 71.147}
        & {295.106}      \\
    ORB-SLAM3           
        & { 28.422}
        & { 48.546}  
        & { 19.828}
        & { - }   \\
    \bf{Odometry + SGF} 
        & { \textbf{9.482}}
        & { \textbf{14.384}}  % 67.625(IPM)
        & { \textbf{12.365}}
        & { \textbf{11.540}}  \\
    % \bf{ORB-SLAM3 + SGF}
    %     & { } 
    %     & { - } 
    %     & {--}  
    %     & { 13.047}     \\
    \bottomrule
\end{tabular}
}
\newline
\caption{Absolute Trajectory Error (ATE). (m)}
\label{tab:trajacc}
\end{table}

\figref{fig:traj_plot} shows how the proposed \ac{SGF} factor performs in a complex campus scenario. The quantitative comparison for this scenario can be found in \tabref{tab:trajacc}. 
For all sequences, We can see that the proposed method achieves a good performance compared to the traditional vision-based method, ORB-SLAM3. For \textit{Seq. Delivery}, both ORB-SLAM3 and the proposed method performed well, but we can see that our proposed method achieved lower errors with reverse loop detection. The \textit{Seq. Reverse + Slope} showed relatively low accuracy among all sequences because the SGFs were extracted from uneven ground. In the \textit{Seq. Large Loop}, ORB-SLAM3 lost tracking while driving. Comparing the trajectory before the tracking loss, we can see that the error was not corrected at the reverse loop point. 
% 모든 시퀀스에서 제안하는 방법이 전통적인 vision-based 방식인 ORB-SLAM3보다 잘 나온것을 확인할 수 있다. delivery 시퀀스에서는 orb-slam3와 posposed 모두 좋은 성능을 보였지만, 제안하는 방법에서 reverse loop closing을 통해 error가 더 적게 나온 것을 볼 수 있다. reverse 시퀀스는 경사가 있는 상황에서 SGF 자체가 고르지 못한 지면에서 추출되기 때문에 전체 시퀀스 중에서는 상대적으로 낮은 정확도를 보여주었다. large loop에서 ORB-SLAM3는 중간에 tracking loss가 발생하였다. 이전까지의 trajectory를 비교해보면 reverse loop가 발생하는 지점에서 오차가 발생하는 것을 확인할 수 있음. 
%\figref{fig:traj_plot:seq_lloop}에서는 넓은 지역을 긴 시간 동안 돌아다니는 시퀀스임. Odometry의 경우 긴 시간 동안 오차가 매우 많이 누적되는 것을 알 수 있고, ORB-SLAM3의 경우 loop detection을 통해 상대적으로 정확한 trajectory를 추출하지만, 다이나믹한 환경에서 주행 도중 tracking lost가 발생하였음. SGF factor를 추가로 사용했을 때, 둘 다 모두 좋은 성능을 보여주었지만, 특히 forward loop가 발생하지 않는 부분에서 ORB SLAM3보다 더 gt에 가까운 위치로 trajectory를 optimize한 것을 알 수 있음. Reverse_Slope은 모든 loop가 reverse로 발생하고, 경사 상황이 많이 발생하는 시퀀스 이다. 이 경우 다른 방법들 보다 ORB-SLAM3자체의 성능을 포함하여 결과가 별로 좋지 않게 나왔다. 이는 MC-IPM을 통해 지면 정보를 robust하게 추출하지만, 그럼에도 불구하고 지면 자체의 마모나 풍화가 많이 돼서 SGF가 큰 역할을 하지 못했기 때문이다. 배달 시퀀스에서는 전체적으로 좋은 결과를 보였음. 그러나 ORB-SLAM3의 경우 z축으로 편향을 가지고 있어 trajectory에 z값 에러가 누적되었는데 SGF를 더했을 때, reverse loop를 통해 error가 줄어는 모습을 확인할 수 있음.

% The proposed method shows the best results with reverse loop closing. Similarly, in the \figref{fig:traj_plot:seq_reverseloop}, the proposed method minimized the drift through reverse loop detection and optimization, while others were shown to accumulate drift.



\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.1} 
\resizebox{\columnwidth}{!}{
    \begin{tabular}{l | c | c | c }
        \toprule
        {Sequences}& {Detection} & {Find loop pairs (Rev.)} & {Loop closed (Rev.)}
        \\
        \hline\hline
        
        Seq. Large Loop      & 79/94  &  33/34 (3/3)  &  31 (1)  \\
        Seq. Reverse+Slope    & 37/46  &  11/16 (11/16) &  7  (7)  \\
        Seq. Delivery        & 19/23  &    1/1 (1/1)  &  1  (1)  \\
          
    \bottomrule
    \end{tabular}
}
\newline\textbf{}
\caption{Quantitative results for \ac{SGF} detector, loop finding, and loop matching in each sequence.}
\label{tab:seq_metrics_result}
\end{table}

% Table3에서 각 열은 seq별로 moment based detection, clustering, 그리고 loop matching에 대한 결과를 정량적으로 보여줍니다. 첫 열은 경로에서 detectio 되어야 하는 전체 개수 대비 찾은 개수, 두 번째 열은 전체 loop pair 중 같은 SGF group에 묶인 pair개수, 마지막 열은 두 번쨰 열에서 얻어진 pair 중 SGF loop matching이 성공한 횟수입니다. 괄호는 reverse 상황을 나타냅니다. 제안된 SGF detector는 거의 80%이상의 검출 성공률을 보였으며, SGF descriptor는reverse 상황에서도 절반 이상에서 loop matching을 성공시켰습니다.
In \tabref{tab:seq_metrics_result}, each column quantitatively shows results for moment-based detection, loop finding, and loop matching by all sequences. The first column is the number of \ac{SGF}s found relative to the total number of \ac{SGF}s that should be detected in the path, the second column is the number of pairs grouped in the same \ac{SGF} group among all loop pairs, and the last column is the number of \ac{SGF} loop matching was successful among the pairs obtained in the second column. Parentheses indicate the reverse loop cases. 
% The proposed moment based detector showed a detection success rate of nearly 80\% or higher, and the \ac{SGF} descriptor succeeded in loop matching in more than half, even in reverse loop cases.
The proposed moment-based detector showed a detection success rate of nearly 80\% or higher, and the \ac{SGF} descriptor succeeded in loop matching in more than half, even in reverse loop cases.


% SGF가 야간에도 낮과 같이 견고한 factor로서 쓰일 수 있는지 검증을 위해 Seq. Large Loop와 동일한 경로로 밤에 데이터 취득을 하였습니다. 당시 로봇의 전방 조명을 이용하였고, 야간 input data에 대해 contrast limited adaptive histogram equalization (CLAHE) 전처리를 적용하였습니다. 지면 이미지는 단순 처리로도 낮과 매우 비슷한 SGF 결과를 얻을 수 있었습니다. 이는 SGF가 어두운 조건에서도 강건하게 작용할 수 있음을 보여줍니다. loop mat전체 결과는 Fig.10 (b)에 나와있습니다.
We also tested the \ac{SGF} for the night-time sequences. Each robot is equipped with LED lights, and we applied Contrast Limited Adaptive Histogram Equalization (CLAHE) to enhance the contrast of dark images. As in \figref{fig:traj_plot}, the proposed method resulted in equivalent performance compared to the daytime. Note that ORB-SLAM 3 failed to optimize for both raw and enhanced night sequences. 

%To verify that \ac{SGF} can be as robust a factor at night as it is during the day, we acquired data at night using the same path as Seq. Large Loop. We used the robot's forward light and applied Contrast Limited Adaptive Histogram Equalization (CLAHE) preprocessing to the night input data. For the ground image, we were able to achieve equivalent performance comparing to the daytime with simple processing, which shows that SGF can be robust in dark conditions. The full results are shown in \figref{fig:traj_plot}.


\subsection{Comparison of \ac{MC-IPM} and \ac{IPM}}
To evaluate the performance of MC-IPM compensation, we quantitatively compare the \ac{ATE} with conventional IPM methods. In uneven ground conditions, the typical IPM cannot provide consistent information to the SGF detector, resulting in poor performance. For a more explicit comparison, we selected two sequences (Seq. Large loop, Seq. Reverse+Slope) with varying ground conditions and a large number of loop pairs. The results are shown in \tabref{tab:MCIPM_IPM_result}.



% MC-IPM 적용 전과 후의 SGF의 개수 차이?
\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.1} 
\resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{l | c | c }
    \toprule
        {Sequences}& {\ac{MC-IPM}} & {IPM}
        \\
        \hline\hline
        
        Seq. Large Loop      &  \textbf{9.482} $(m)$  &  12.567 $(m)$ \\
        Seq. Reverse+Slope   &  \textbf{14.384} $(m)$  &  67.625 $(m)$ \\
        % Seq. Delivery        &  -  &  -  \\
          
    \bottomrule
    \end{tabular}
}
\newline\textbf{}
.\caption{Comparison \ac{ATE} of \ac{MC-IPM} and \ac{IPM}.}
\label{tab:MCIPM_IPM_result}
\end{table}

















% % ============================= Template =======================================================
% In Table \ref{tab:trajacc}, shows ATE, RTE of Odometry, ORB-SLAM3 (Mono-IMU), Proposed.

% \begin{table}[h]
% \centering
% \begin{tabular}{l c c c}
%     \toprule
%     \multicolumn{4}{c}{F1-accuracy} 
% \\
%     \midrule
%     {Methods}
%     & {sequence 1}
%     & {sequence 2}
%     & {sequence 3}
% \\
%     \midrule
%     \bf{Odometry}       & {--}  & {--}  & {--}     \\
%     \bf{Odometry+SGF}   & {--}  & {--}  & {--}  \\
%     \bf{ORB-SLAM3}      & {--}  & {--}  & {--}   \\
%     \midrule
%     \textbf{sixth}  &  0.89   &  0.686  &  0.873 \\
%     \bottomrule
% \end{tabular}
% \newline
% \caption{Result APE/RPE of proposed method}
% \label{tab:trajacc}
% \end{table}

% -----------------------------------------------------------------------------------
% Table3은 각 seq에서 moment based detection과 loop pa 그리고 loop closing 성공 횟수를 정량적으로 보여줍니다. 




%% =======IPM Result ======================================================
% \begin{figure*}[t]
% \centering
% % \begin{TAB}[2pt]{c|cccc|c|c}{|c|c|c|}% (rows,min,max)[tabsep]{columns}{rows}
% \begin{tabular}{c c c c c c c}%{c|c c c c|c|c}
%     \bf{IPM} & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/001083.png}\end{minipage}
%             & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/001090.png}\end{minipage}
%             & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/001094.png}\end{minipage}
%             & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/001098.png}\end{minipage} 
%             & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/000321.png}\end{minipage}
%             & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/000321.png}\end{minipage}
% \vspace{5pt}
% \\ 
%     \bf{MC-IPM} & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/001083.png}\end{minipage}
%     & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/001090.png}\end{minipage}
%     & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/001094.png}\end{minipage}
%     & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/001098.png}\end{minipage} 
%     & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/000321.png}\end{minipage}
%     & \begin{minipage}{0.12\textwidth}\includegraphics[width=\linewidth]{assets/000321.png}\end{minipage}
% \vspace{5pt}
% \\
%     & \multicolumn{4}{c}{bump} & up hill & down hill     
% \end{tabular}
% \caption{MC-IPM result}
% \label{fig:mcipm}
% \end{figure*}

==> admin/initial_latex/5_Conclusion.tex <==
\section{Conclusion}

% 본 논문에서는 표준 마킹과 복잡한 도심 구조의 특성 중 하나인 man-made feature를 통합하여 SGF로써 활용하는 새로운 localization 시스템을 제안합니다. 불규칙적인 지형 조건에서 보다 일관적인 SGF를 얻기 위해 로봇의 모션을 이용하는 MC-IPM을 적용했습니다. SGF factor는 실제 운용되는 배달 로봇에 적용되어 캠퍼스 환경에서 좋은 성능을 보였으며 reverse loop case를 해결할 수 있었습니다. 또한 낮과 밤을 통틀어 조명 변화 및 외관 변화에도 강력한 성능을 보였습니다.
% 이후 연구는 SGF를 비전 기반 SLAM 알고리즘에 통합하여 더 좋은 성능을 내는 방법론을 구축하는 것입니다.


In this paper, we propose a novel localization system that integrates standard markings and man-made features, one of the characteristics of complex urban structures, and utilizes them as SGF. To obtain more consistent \ac{SGF} under uneven terrain conditions, we applied \ac{MC-IPM}, which utilizes the robot's motion. The \ac{SGF} factor was applied to a live delivery robot, performing well in the campus environment and solving the reverse loop case. It also validated strong performance against changes in lighting and appearance throughout the day and night.
Our future work is to build a methodology that integrates \ac{SGF} into vision-based SLAM algorithms to perform better.
